Scaleformer: Iterative Multi-scale Refining Transformers for Time Series Forecasting

The performance of time series forecasting has recently been greatly improved by the introduction of transformers. In this paper, we propose a general multi-scale framework that can be applied to the state-of-the-art transformer-based time series forecasting models (FEDformer, Autoformer, etc.). By iteratively refining a forecasted time series at multiple scales with shared weights, introducing architecture adaptations, and a specially-designed normalization scheme, we are able to achieve significant performance improvements, from 5.5% to 38.5% across datasets and transformer architectures, with minimal additional computational overhead. Via detailed ablation studies, we demonstrate the effectiveness of each of our contributions across the architecture and methodology. Furthermore, our experiments on various public datasets demonstrate that the proposed improvements outperform their corresponding baseline counterparts. Our code is publicly available in https://github.com/BorealisAI/scaleformer.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/ablation_autoformer.tex <==
\begin{table}
\scriptsize	  
	\centering
	\caption{Comparison of Autoformer model using multi-scale framework with MSE loss for training "-MS" and Adaptive loss "-MSA". As we can see, the combination of all our proposed contributions is essential, and results in significantly improved performance.}
	\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{Autoformer-A} & \multicolumn{2}{c}{Autoformer-MS} &  \multicolumn{2}{c}{Autoformer-MSA}\\ 
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
 & 96 & 0.267\scalebox{0.8}{$\pm$0.03} & 0.334\scalebox{0.8}{$\pm$0.02} & 0.229\scalebox{0.8}{$\pm$0.01} & 0.288\scalebox{0.8}{$\pm$0.01} & \underline{0.174}\scalebox{0.8}{$\pm$0.01} & \underline{0.254}\scalebox{0.8}{$\pm$0.01} & \textbf{0.163}\scalebox{0.8}{$\pm$0.01} & \textbf{0.226}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.323\scalebox{0.8}{$\pm$0.01} & 0.376\scalebox{0.8}{$\pm$0.00} & 0.293\scalebox{0.8}{$\pm$0.02} & 0.340\scalebox{0.8}{$\pm$0.02} & \underline{0.250}\scalebox{0.8}{$\pm$0.02} & \underline{0.333}\scalebox{0.8}{$\pm$0.02} & \textbf{0.221}\scalebox{0.8}{$\pm$0.01} & \textbf{0.290}\scalebox{0.8}{$\pm$0.02} \\ 
 & 336 & 0.364\scalebox{0.8}{$\pm$0.02} & 0.397\scalebox{0.8}{$\pm$0.01} & 0.357\scalebox{0.8}{$\pm$0.01} & 0.387\scalebox{0.8}{$\pm$0.01} & \underline{0.314}\scalebox{0.8}{$\pm$0.02} & \underline{0.380}\scalebox{0.8}{$\pm$0.02} & \textbf{0.282}\scalebox{0.8}{$\pm$0.02} & \textbf{0.340}\scalebox{0.8}{$\pm$0.03} \\ 
 & 720 & 0.425\scalebox{0.8}{$\pm$0.01} & 0.434\scalebox{0.8}{$\pm$0.01} & 0.419\scalebox{0.8}{$\pm$0.01} & \underline{0.422}\scalebox{0.8}{$\pm$0.01} & \underline{0.414}\scalebox{0.8}{$\pm$0.03} & 0.457\scalebox{0.8}{$\pm$0.02} & \textbf{0.369}\scalebox{0.8}{$\pm$0.04} & \textbf{0.396}\scalebox{0.8}{$\pm$0.03} \\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
 & 96 & 0.197\scalebox{0.8}{$\pm$0.01} & \underline{0.312}\scalebox{0.8}{$\pm$0.01} & 0.201\scalebox{0.8}{$\pm$0.01} & 0.312\scalebox{0.8}{$\pm$0.01} & \underline{0.196}\scalebox{0.8}{$\pm$0.00} & 0.312\scalebox{0.8}{$\pm$0.01} & \textbf{0.188}\scalebox{0.8}{$\pm$0.00} & \textbf{0.303}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.219\scalebox{0.8}{$\pm$0.01} & 0.329\scalebox{0.8}{$\pm$0.01} & 0.221\scalebox{0.8}{$\pm$0.01} & 0.328\scalebox{0.8}{$\pm$0.01} & \underline{0.208}\scalebox{0.8}{$\pm$0.00} & \underline{0.323}\scalebox{0.8}{$\pm$0.00} & \textbf{0.197}\scalebox{0.8}{$\pm$0.00} & \textbf{0.310}\scalebox{0.8}{$\pm$0.00} \\ 
 & 336 & 0.263\scalebox{0.8}{$\pm$0.04} & 0.359\scalebox{0.8}{$\pm$0.03} & 0.232\scalebox{0.8}{$\pm$0.01} & 0.339\scalebox{0.8}{$\pm$0.01} & \textbf{0.220}\scalebox{0.8}{$\pm$0.00} & \underline{0.336}\scalebox{0.8}{$\pm$0.00} & \underline{0.224}\scalebox{0.8}{$\pm$0.02} & \textbf{0.333}\scalebox{0.8}{$\pm$0.01} \\ 
 & 720 & 0.290\scalebox{0.8}{$\pm$0.05} & 0.380\scalebox{0.8}{$\pm$0.02} & \textbf{0.249}\scalebox{0.8}{$\pm$0.01} & \textbf{0.351}\scalebox{0.8}{$\pm$0.01} & 0.252\scalebox{0.8}{$\pm$0.00} & 0.364\scalebox{0.8}{$\pm$0.00} & \underline{0.249}\scalebox{0.8}{$\pm$0.01} & \underline{0.358}\scalebox{0.8}{$\pm$0.01} \\
    \bottomrule
	\end{tabular}
    \label{table:ablation_autoformer}
\end{table}

==> tables/ablation_informer.tex <==
\begin{table}
  \scriptsize	  
	\centering
	\caption{Comparison of Informer model using multi-scale framework with MSE loss for training "-MS" and Adaptive loss "-MSA". As we can see, the combination of all our proposed contributions is essential, and results in significantly improved performance.}
	\label{tab:ablation}
	\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{Informer-A} & \multicolumn{2}{c}{Informer-MS} &  \multicolumn{2}{c}{Informer-MSA}\\ 
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
 & 96 & 0.388\scalebox{0.8}{$\pm$0.04} & 0.435\scalebox{0.8}{$\pm$0.03} & 0.342\scalebox{0.8}{$\pm$0.03} & 0.382\scalebox{0.8}{$\pm$0.02} & \underline{0.249}\scalebox{0.8}{$\pm$0.02} & \underline{0.324}\scalebox{0.8}{$\pm$0.01} & \textbf{0.210}\scalebox{0.8}{$\pm$0.02} & \textbf{0.279}\scalebox{0.8}{$\pm$0.02} \\ 
 & 192 & 0.433\scalebox{0.8}{$\pm$0.05} & 0.453\scalebox{0.8}{$\pm$0.03} & 0.385\scalebox{0.8}{$\pm$0.02} & 0.404\scalebox{0.8}{$\pm$0.01} & \underline{0.315}\scalebox{0.8}{$\pm$0.02} & \underline{0.380}\scalebox{0.8}{$\pm$0.02} & \textbf{0.289}\scalebox{0.8}{$\pm$0.01} & \textbf{0.333}\scalebox{0.8}{$\pm$0.01} \\ 
 & 336 & 0.610\scalebox{0.8}{$\pm$0.04} & 0.551\scalebox{0.8}{$\pm$0.02} & 0.656\scalebox{0.8}{$\pm$0.10} & 0.550\scalebox{0.8}{$\pm$0.04} & \underline{0.473}\scalebox{0.8}{$\pm$0.04} & \underline{0.478}\scalebox{0.8}{$\pm$0.02} & \textbf{0.418}\scalebox{0.8}{$\pm$0.04} & \textbf{0.427}\scalebox{0.8}{$\pm$0.03} \\ 
 & 720 & 0.978\scalebox{0.8}{$\pm$0.05} & 0.723\scalebox{0.8}{$\pm$0.02} & 0.953\scalebox{0.8}{$\pm$0.04} & 0.680\scalebox{0.8}{$\pm$0.02} & \underline{0.664}\scalebox{0.8}{$\pm$0.04} & \underline{0.585}\scalebox{0.8}{$\pm$0.02} & \textbf{0.595}\scalebox{0.8}{$\pm$0.04} & \textbf{0.532}\scalebox{0.8}{$\pm$0.02} \\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
 & 96 & 0.344\scalebox{0.8}{$\pm$0.00} & 0.421\scalebox{0.8}{$\pm$0.00} & 0.321\scalebox{0.8}{$\pm$0.00} & 0.402\scalebox{0.8}{$\pm$0.00} & \underline{0.211}\scalebox{0.8}{$\pm$0.00} & \underline{0.326}\scalebox{0.8}{$\pm$0.00} & \textbf{0.203}\scalebox{0.8}{$\pm$0.01} & \textbf{0.315}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.344\scalebox{0.8}{$\pm$0.01} & 0.426\scalebox{0.8}{$\pm$0.01} & 0.341\scalebox{0.8}{$\pm$0.01} & 0.422\scalebox{0.8}{$\pm$0.01} & \underline{0.233}\scalebox{0.8}{$\pm$0.01} & \underline{0.348}\scalebox{0.8}{$\pm$0.00} & \textbf{0.219}\scalebox{0.8}{$\pm$0.00} & \textbf{0.331}\scalebox{0.8}{$\pm$0.00} \\ 
 & 336 & 0.358\scalebox{0.8}{$\pm$0.01} & 0.440\scalebox{0.8}{$\pm$0.01} & 0.344\scalebox{0.8}{$\pm$0.00} & 0.422\scalebox{0.8}{$\pm$0.00} & \underline{0.279}\scalebox{0.8}{$\pm$0.01} & \underline{0.388}\scalebox{0.8}{$\pm$0.01} & \textbf{0.253}\scalebox{0.8}{$\pm$0.01} & \textbf{0.360}\scalebox{0.8}{$\pm$0.01} \\ 
 & 720 & 0.386\scalebox{0.8}{$\pm$0.00} & 0.452\scalebox{0.8}{$\pm$0.00} & 0.363\scalebox{0.8}{$\pm$0.00} & 0.432\scalebox{0.8}{$\pm$0.00} & \underline{0.315}\scalebox{0.8}{$\pm$0.01} & \underline{0.411}\scalebox{0.8}{$\pm$0.00} & \textbf{0.293}\scalebox{0.8}{$\pm$0.01} & \textbf{0.390}\scalebox{0.8}{$\pm$0.01} \\ 
    \bottomrule
	\end{tabular}
    \label{table:ablation_informer}
\end{table}

==> tables/ablation_joint.tex <==
\begin{table}
  \scriptsize	  
	\centering
	\caption{Comparison of training with Adaptive loss "-\textbf{A}", multi-scale framework with MSE loss "-\textbf{MS}", Multi-scale framework and Adaptive loss "-\textbf{MSA}". It shows the combination of all our proposed contributions is essential, and results in significantly improved performance.}
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{Informer-\textbf{A}} & \multicolumn{2}{c}{Informer-\textbf{MS}} &  \multicolumn{2}{c}{Informer-\textbf{MSA}}\\ 
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
 & 96 & 0.388\scalebox{0.8}{$\pm$0.04} & 0.435\scalebox{0.8}{$\pm$0.03} & 0.342\scalebox{0.8}{$\pm$0.03} & 0.382\scalebox{0.8}{$\pm$0.02} & 0.249\scalebox{0.8}{$\pm$0.02} & 0.324\scalebox{0.8}{$\pm$0.01} & \textbf{0.210}\scalebox{0.8}{$\pm$0.02} & \textbf{0.279}\scalebox{0.8}{$\pm$0.02} \\ 
 & 192 & 0.433\scalebox{0.8}{$\pm$0.05} & 0.453\scalebox{0.8}{$\pm$0.03} & 0.385\scalebox{0.8}{$\pm$0.02} & 0.404\scalebox{0.8}{$\pm$0.01} & 0.315\scalebox{0.8}{$\pm$0.02} & 0.380\scalebox{0.8}{$\pm$0.02} & \textbf{0.289}\scalebox{0.8}{$\pm$0.01} & \textbf{0.333}\scalebox{0.8}{$\pm$0.01} \\ 
 & 336 & 0.610\scalebox{0.8}{$\pm$0.04} & 0.551\scalebox{0.8}{$\pm$0.02} & 0.656\scalebox{0.8}{$\pm$0.10} & 0.550\scalebox{0.8}{$\pm$0.04} & 0.473\scalebox{0.8}{$\pm$0.04} & 0.478\scalebox{0.8}{$\pm$0.02} & \textbf{0.418}\scalebox{0.8}{$\pm$0.04} & \textbf{0.427}\scalebox{0.8}{$\pm$0.03} \\ 
 & 720 & 0.978\scalebox{0.8}{$\pm$0.05} & 0.723\scalebox{0.8}{$\pm$0.02} & 0.953\scalebox{0.8}{$\pm$0.04} & 0.680\scalebox{0.8}{$\pm$0.02} & 0.664\scalebox{0.8}{$\pm$0.04} & 0.585\scalebox{0.8}{$\pm$0.02} & \textbf{0.595}\scalebox{0.8}{$\pm$0.04} & \textbf{0.532}\scalebox{0.8}{$\pm$0.02} \\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
 & 96 & 0.344\scalebox{0.8}{$\pm$0.00} & 0.421\scalebox{0.8}{$\pm$0.00} & 0.321\scalebox{0.8}{$\pm$0.00} & 0.402\scalebox{0.8}{$\pm$0.00} & 0.211\scalebox{0.8}{$\pm$0.00} & 0.326\scalebox{0.8}{$\pm$0.00} & \textbf{0.203}\scalebox{0.8}{$\pm$0.01} & \textbf{0.315}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.344\scalebox{0.8}{$\pm$0.01} & 0.426\scalebox{0.8}{$\pm$0.01} & 0.341\scalebox{0.8}{$\pm$0.01} & 0.422\scalebox{0.8}{$\pm$0.01} & 0.233\scalebox{0.8}{$\pm$0.01} & 0.348\scalebox{0.8}{$\pm$0.00} & \textbf{0.219}\scalebox{0.8}{$\pm$0.00} & \textbf{0.331}\scalebox{0.8}{$\pm$0.00} \\ 
 & 336 & 0.358\scalebox{0.8}{$\pm$0.01} & 0.440\scalebox{0.8}{$\pm$0.01} & 0.344\scalebox{0.8}{$\pm$0.00} & 0.422\scalebox{0.8}{$\pm$0.00} & 0.279\scalebox{0.8}{$\pm$0.01} & 0.388\scalebox{0.8}{$\pm$0.01} & \textbf{0.253}\scalebox{0.8}{$\pm$0.01} & \textbf{0.360}\scalebox{0.8}{$\pm$0.01} \\ 
 & 720 & 0.386\scalebox{0.8}{$\pm$0.00} & 0.452\scalebox{0.8}{$\pm$0.00} & 0.363\scalebox{0.8}{$\pm$0.00} & 0.432\scalebox{0.8}{$\pm$0.00} & 0.315\scalebox{0.8}{$\pm$0.01} & 0.411\scalebox{0.8}{$\pm$0.00} & \textbf{0.293}\scalebox{0.8}{$\pm$0.01} & \textbf{0.390}\scalebox{0.8}{$\pm$0.01} \\ 
    \bottomrule
	\end{tabular}}

\vspace{0.3cm}
\scriptsize	  
	\centering
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{Autoformer-\textbf{A}} & \multicolumn{2}{c}{Autoformer-\textbf{MS}} &  \multicolumn{2}{c}{Autoformer-\textbf{MSA}}\\ 
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
 & 96 & 0.267\scalebox{0.8}{$\pm$0.03} & 0.334\scalebox{0.8}{$\pm$0.02} & 0.229\scalebox{0.8}{$\pm$0.01} & 0.288\scalebox{0.8}{$\pm$0.01} & 0.174\scalebox{0.8}{$\pm$0.01} & 0.254\scalebox{0.8}{$\pm$0.01} & \textbf{0.163}\scalebox{0.8}{$\pm$0.01} & \textbf{0.226}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.323\scalebox{0.8}{$\pm$0.01} & 0.376\scalebox{0.8}{$\pm$0.00} & 0.293\scalebox{0.8}{$\pm$0.02} & 0.340\scalebox{0.8}{$\pm$0.02} & 0.250\scalebox{0.8}{$\pm$0.02} & 0.333\scalebox{0.8}{$\pm$0.02} & \textbf{0.221}\scalebox{0.8}{$\pm$0.01} & \textbf{0.290}\scalebox{0.8}{$\pm$0.02} \\ 
 & 336 & 0.364\scalebox{0.8}{$\pm$0.02} & 0.397\scalebox{0.8}{$\pm$0.01} & 0.357\scalebox{0.8}{$\pm$0.01} & 0.387\scalebox{0.8}{$\pm$0.01} & 0.314\scalebox{0.8}{$\pm$0.02} & 0.380\scalebox{0.8}{$\pm$0.02} & \textbf{0.282}\scalebox{0.8}{$\pm$0.02} & \textbf{0.340}\scalebox{0.8}{$\pm$0.03} \\ 
 & 720 & 0.425\scalebox{0.8}{$\pm$0.01} & 0.434\scalebox{0.8}{$\pm$0.01} & 0.419\scalebox{0.8}{$\pm$0.01} & 0.422\scalebox{0.8}{$\pm$0.01} & 0.414\scalebox{0.8}{$\pm$0.03} & 0.457\scalebox{0.8}{$\pm$0.02} & \textbf{0.369}\scalebox{0.8}{$\pm$0.04} & \textbf{0.396}\scalebox{0.8}{$\pm$0.03} \\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
 & 96 & 0.197\scalebox{0.8}{$\pm$0.01} & 0.312\scalebox{0.8}{$\pm$0.01} & 0.201\scalebox{0.8}{$\pm$0.01} & 0.312\scalebox{0.8}{$\pm$0.01} & 0.196\scalebox{0.8}{$\pm$0.00} & 0.312\scalebox{0.8}{$\pm$0.01} & \textbf{0.188}\scalebox{0.8}{$\pm$0.00} & \textbf{0.303}\scalebox{0.8}{$\pm$0.01} \\ 
 & 192 & 0.219\scalebox{0.8}{$\pm$0.01} & 0.329\scalebox{0.8}{$\pm$0.01} & 0.221\scalebox{0.8}{$\pm$0.01} & 0.328\scalebox{0.8}{$\pm$0.01} & 0.208\scalebox{0.8}{$\pm$0.00} & 0.323\scalebox{0.8}{$\pm$0.00} & \textbf{0.197}\scalebox{0.8}{$\pm$0.00} & \textbf{0.310}\scalebox{0.8}{$\pm$0.00} \\ 
 & 336 & 0.263\scalebox{0.8}{$\pm$0.04} & 0.359\scalebox{0.8}{$\pm$0.03} & 0.232\scalebox{0.8}{$\pm$0.01} & 0.339\scalebox{0.8}{$\pm$0.01} & \textbf{0.220}\scalebox{0.8}{$\pm$0.00} & 0.336\scalebox{0.8}{$\pm$0.00} & 0.224\scalebox{0.8}{$\pm$0.02} & \textbf{0.333}\scalebox{0.8}{$\pm$0.01} \\ 
 & 720 & 0.290\scalebox{0.8}{$\pm$0.05} & 0.380\scalebox{0.8}{$\pm$0.02} & \textbf{0.249}\scalebox{0.8}{$\pm$0.01} & \textbf{0.351}\scalebox{0.8}{$\pm$0.01} & 0.252\scalebox{0.8}{$\pm$0.00} & 0.364\scalebox{0.8}{$\pm$0.00} & 0.249\scalebox{0.8}{$\pm$0.01} & 0.358\scalebox{0.8}{$\pm$0.01} \\
    \bottomrule
	\end{tabular}} % scalebox
    \label{tab:ablation_joint}
\end{table}

==> tables/main_results.tex <==
\begin{table}
\setlength\tabcolsep{2pt}
\footnotesize	
	\centering
	\caption{Comparison of the MSE and MAE results for our proposed multi-scale framework version of different methods (-\textbf{MSA}) with their original models as the baseline. Results are given in the \emph{multi-variate} setting, for different lenghts of the horizon window. The look-back window size is fixed to $96$ for all experiments. The best results are shown in \textbf{Bold}. Our method outperforms vanilla versions of the baselines over almost all datasets and settings. The numbers at the end of each row report the average improvement of scaleformer over the baseline.\lili{either transpose or put in the table?}}
	\scalebox{0.85}{\begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc|cccc} 
% 		\toprule
		\cmidrule(lr){1-22}\morecmidrules\cmidrule(lr){1-22}
		\multirow{2}{*}{Method} & \multirow{2}{*}{Metric} & \multicolumn{4}{c|}{Exchange} & \multicolumn{4}{c|}{Weather} &  \multicolumn{4}{c|}{Electricity} &  \multicolumn{4}{c|}{Traffic} &  \multicolumn{4}{c|}{ILI} &
		\multicolumn{4}{c}{\textcolor{green}{\bold{Improvement}}}\\ 
% 		\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18} \cmidrule(lr){19-22}
		& & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 24 & 32 & 48 & 64 \\
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{FED} 
 & MSE & 0.155 & 0.274 & \textbf{0.452} & \textbf{1.172} & 0.288 & 0.368 & \textbf{0.447} & \textbf{0.640} & 0.201 & 0.200 & 0.214 & 0.239 & 0.601 & 0.603 & 0.602 & 0.615 & 3.025 & 3.034 & \textbf{2.444} & 2.686 \\ 
 & MAE & 0.285 & 0.384 & \textbf{0.498} & \textbf{0.839} & 0.365 & 0.425 & 0.469 & 0.574 & 0.317 & 0.314 & 0.330 & 0.350 & 0.376 & 0.379 & 0.375 & 0.378 & 1.189 & 1.201 & \textbf{1.041} & 1.112 \\ 
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{FED-MSA} 
 & MSE & \textbf{0.109} & \textbf{0.241} & 0.471 & 1.259 & \textbf{0.220} & \textbf{0.341} & 0.463 & 0.682 & \textbf{0.182} & \textbf{0.188} & \textbf{0.210} & \textbf{0.232} & \textbf{0.564} & \textbf{0.570} & \textbf{0.576} & \textbf{0.602} & \textbf{2.745} & \textbf{2.748} & 2.793 & \textbf{2.678} & {\color{green}5.57\%} \\ 
 & MAE & \textbf{0.240} & \textbf{0.353} & 0.508 & 0.865 & \textbf{0.289} & \textbf{0.385} & \textbf{0.455} & \textbf{0.565} & \textbf{0.297} & \textbf{0.300} & \textbf{0.324} & \textbf{0.339} & \textbf{0.351} & \textbf{0.349} & \textbf{0.349} & \textbf{0.360} & \textbf{1.075} & \textbf{1.072} & 1.059 & \textbf{1.071} & {\color{green}5.93\%} \\ 

\cmidrule(lr){1-22}%\morecmidrules\cmidrule(lr){1-22}
% \midrule
% \midrule

\multirow{2}{*}{AUTO} 
 & MSE & 0.154 & 0.356 & \textbf{0.441} & 1.118 & 0.267 & 0.323 & 0.364 & 0.425 & 0.197 & 0.219 & 0.263 & 0.290 & 0.628 & 0.634 & 0.619 & 0.656 & 3.862 & 3.871 & \textbf{2.891} & 3.164 \\ 
 & MAE & 0.285 & 0.428 & \textbf{0.495} & 0.819 & 0.334 & 0.376 & 0.397 & 0.434 & 0.312 & 0.329 & 0.359 & 0.380 & 0.393 & 0.401 & 0.385 & 0.403 & 1.370 & 1.379 & \textbf{1.138} & 1.223 \\ 
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{AUTO-MSA} 
 & MSE & \textbf{0.126} & \textbf{0.253} & 0.519 & \textbf{0.928} & \textbf{0.163} & \textbf{0.221} & \textbf{0.282} & \textbf{0.369} & \textbf{0.188} & \textbf{0.197} & \textbf{0.224} & \textbf{0.249} & \textbf{0.567} & \textbf{0.589} & \textbf{0.619} & \textbf{0.642} & \textbf{3.370} & \textbf{3.088} & 3.207 & \textbf{2.954} & {\color{green}13.48\%}\\ 
 & MAE & \textbf{0.259} & \textbf{0.373} & 0.538 & \textbf{0.751} & \textbf{0.226} & \textbf{0.290} & \textbf{0.340} & \textbf{0.396} & \textbf{0.303} & \textbf{0.310} & \textbf{0.333} & \textbf{0.358} & \textbf{0.350} & \textbf{0.360} & \textbf{0.383} & \textbf{0.397} & \textbf{1.213} & \textbf{1.164} & 1.153 & \textbf{1.112} & {\color{green}9.08\%} \\ 

\cmidrule(lr){1-22}%\morecmidrules\cmidrule(lr){1-22}
% \midrule
% \midrule

\multirow{2}{*}{Info}
 & MSE & 0.966 & 1.088 & 1.598 & 2.679 & 0.388 & 0.433 & 0.610 & 0.978 & 0.344 & 0.344 & 0.358 & 0.386 & 0.748 & 0.772 & 0.868 & 1.074 & 5.402 & 5.296 & 5.226 & 5.304 \\ 
 & MAE & 0.792 & 0.842 & 1.016 & 1.340 & 0.435 & 0.453 & 0.551 & 0.723 & 0.421 & 0.426 & 0.440 & 0.452 & 0.426 & 0.436 & 0.493 & 0.606 & 1.581 & 1.587 & 1.569 & 1.578 \\ 
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{Info-MSA} 
 & MSE & \textbf{0.168} & \textbf{0.427} & \textbf{0.500} & \textbf{1.017} & \textbf{0.210} & \textbf{0.289} & \textbf{0.418} & \textbf{0.595} & \textbf{0.203} & \textbf{0.219} & \textbf{0.253} & \textbf{0.293} & \textbf{0.597} & \textbf{0.655} & \textbf{0.761} & \textbf{0.924} & \textbf{3.742} & \textbf{3.807} & \textbf{3.940} & \textbf{3.670}  & {\color{green}38.52\%}\\ 
 & MAE & \textbf{0.298} & \textbf{0.484} & \textbf{0.535} & \textbf{0.790} & \textbf{0.279} & \textbf{0.333} & \textbf{0.427} & \textbf{0.532} & \textbf{0.315} & \textbf{0.331} & \textbf{0.360} & \textbf{0.390} & \textbf{0.369} & \textbf{0.399} & \textbf{0.455} & \textbf{0.521} & \textbf{1.252} & \textbf{1.272} & \textbf{1.272} & \textbf{1.234} & {\color{green}26.71\%} \\

\cmidrule(lr){1-22}%\morecmidrules\cmidrule(lr){1-22}
% \midrule
% \midrule

\multirow{2}{*}{REF} 
 & MSE & 1.063 & 1.597 & 1.712 & 1.918 & 0.347 & 0.463 & 0.734 & 0.815 & 0.294 & 0.331 & 0.361 & 0.316 & 0.698 & 0.694 & 0.695 & 0.692 & 3.961 & 4.022 & 4.269 & 4.370 \\ 
 & MAE & 0.826 & 1.029 & 1.070 & 1.160 & 0.388 & 0.469 & 0.622 & 0.674 & 0.382 & 0.409 & 0.428 & 0.393 & 0.386 & 0.378 & 0.377 & 0.376 & 1.289 & 1.311 & 1.340 & 1.385 \\ 
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{REF-MSA} 
 & MSE & \textbf{0.182} & \textbf{0.375} & \textbf{0.605} & \textbf{1.089} & \textbf{0.199} & \textbf{0.294} & \textbf{0.463} & \textbf{0.493} & \textbf{0.183} & \textbf{0.194} & \textbf{0.209} & \textbf{0.234} & \textbf{0.615} & \textbf{0.613} & \textbf{0.617} & \textbf{0.638} & \textbf{3.534} & \textbf{3.652} & \textbf{3.506} & \textbf{3.487} & {\color{green} 38.26\%}\\ 
 & MAE & \textbf{0.311} & \textbf{0.446} & \textbf{0.591} & \textbf{0.857} & \textbf{0.263} & \textbf{0.355} & \textbf{0.464} & \textbf{0.471} & \textbf{0.291} & \textbf{0.304} & \textbf{0.321} & \textbf{0.340} & \textbf{0.377} & \textbf{0.367} & \textbf{0.360} & \textbf{0.360} & \textbf{1.212} & \textbf{1.235} & \textbf{1.168} & \textbf{1.177} & {\color{green}25.24\%} \\

\cmidrule(lr){1-22}%\morecmidrules\cmidrule(lr){1-22}
% \midrule
% \midrule

\multirow{2}{*}{PER} 
 & MSE & 0.667 & 1.339 & 1.081 & \textbf{0.867} & 0.441 & 0.475 & 0.478 & \textbf{0.563} & 0.294 & 0.305 & 0.331 & 0.304 & 0.730 & 0.698 & 0.678 & 0.672 & 4.806 & 4.669 & 4.488 & 4.607 \\ 
 & MAE & 0.669 & 0.904 & 0.844 & \textbf{0.766} & 0.479 & 0.501 & 0.482 & \textbf{0.552} & 0.387 & 0.400 & 0.416 & 0.386 & 0.405 & 0.387 & 0.370 & 0.364 & 1.471 & 1.455 & 1.371 & 1.404 \\ 
% \midrule
\cmidrule(lr){1-22}
\multirow{2}{*}{PER-MSA} 
 & MSE & \textbf{0.179} & \textbf{0.439} & \textbf{0.563} & 1.219 & \textbf{0.228} & \textbf{0.302} & \textbf{0.441} & 0.817 & \textbf{0.190} & \textbf{0.200} & \textbf{0.209} & \textbf{0.228} & \textbf{0.612} & \textbf{0.608} & \textbf{0.604} & \textbf{0.634} & \textbf{3.437} & \textbf{3.646} & \textbf{4.055} & \textbf{3.828} & {\color{green} 23.25\%}\\ 
 & MAE & \textbf{0.305} & \textbf{0.486} & \textbf{0.577} & 0.882 & \textbf{0.291} & \textbf{0.357} & \textbf{0.456} & 0.655 & \textbf{0.300} & \textbf{0.310} & \textbf{0.322} & \textbf{0.335} & \textbf{0.371} & \textbf{0.368} & \textbf{0.356} & \textbf{0.360} & \textbf{1.148} & \textbf{1.186} & \textbf{1.248} & \textbf{1.224} & {\color{green}16.92\%} \\ 
%  \bottomrule
\cmidrule(lr){1-22}\morecmidrules\cmidrule(lr){1-22}
	\end{tabular}} % scalebox
    \label{table:ms_final}
\end{table}  

==> tables_rebuttal/illness_dataset.tex <==
\begin{table}
\scriptsize	
	\centering
	\caption{The comparison of the Reformer, Performer, and FEDformer using ILI dataset. For each baseline, our multi-scale framework version is shown with \textbf{-MSA}. For Autoformer and Informer results, please refer to Table 3.}
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Reformer-\textbf{MSA}} & \multicolumn{2}{c}{Performer} &  \multicolumn{2}{c}{Performer-\textbf{MSA}} &  \multicolumn{2}{c}{FEDformer} & \multicolumn{2}{c}{FEDformer-\textbf{MSA}}\\
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MAE & MSE & MAE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{ILI} 
 & 24 & 3.961 & 1.289 & \textbf{3.534} & \textbf{1.212} & 4.806 & 1.471 & \textbf{3.437} & \textbf{1.148} & 3.025 & 1.189 & \textbf{2.745} & \textbf{1.075} \\ 
 & 32 & 4.022 & 1.311 & \textbf{3.652} & \textbf{1.235} & 4.669 & 1.455 & \textbf{3.646} & \textbf{1.186} & 3.034 & 1.201 & \textbf{2.748} & \textbf{1.072} \\ 
 & 48 & 4.269 & 1.340 & \textbf{3.506} & \textbf{1.168} & 4.488 & 1.371 & \textbf{4.055} & \textbf{1.248} & \textbf{2.444} & \textbf{1.041} & 2.793 & 1.059 \\ 
 & 64 & 4.370 & 1.385 & \textbf{3.487} & \textbf{1.177} & 4.607 & 1.404 & \textbf{3.828} & \textbf{1.224} & 2.686 & 1.112 & \textbf{2.678} & \textbf{1.071} \\ 

\bottomrule
	\end{tabular}}
    \label{table:illness_dataset1}
\end{table} 

\begin{table}
\scriptsize	
	\centering
	\caption{Extension of Table 2 for Autoformer and Informer.}
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{Autoformer-\textbf{MSA}} & \multicolumn{2}{c}{Informer} &  \multicolumn{2}{c}{Informer-\textbf{MSA}}\\
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
		\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{ILI} 
 & 24 & 3.862 & 1.370 & \textbf{3.370} & \textbf{1.213} & 5.402 & 1.581 & \textbf{3.742} & \textbf{1.252} \\ 
 & 32 & 3.871 & 1.379 & \textbf{3.088} & \textbf{1.164} & 5.296 & 1.587 & \textbf{3.807} & \textbf{1.272} \\ 
 & 48 & \textbf{2.891} & \textbf{1.138} & 3.207 & 1.153 & 5.226 & 1.569 & \textbf{3.940} & \textbf{1.272} \\ 
 & 64 & 3.164 & 1.223 & \textbf{2.954} & \textbf{1.112} & 5.304 & 1.578 & \textbf{3.670} & \textbf{1.234} \\
\bottomrule
	\end{tabular}}
    \label{table:illness_dataset2}
\end{table}

==> tables_rebuttal/last_value_forecasting.tex <==
\begin{table}
% \setlength{\tabcolsep}{4.5pt}
\scriptsize	
	\centering
	\caption{Last value forecasting baseline for comparison with recent methods}.
	\vspace{+2mm}
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{1}{c}{Output Length\footnote{Output length in parentheses are for ILI dataset.}} & \multicolumn{2}{c}{Exchange} &  \multicolumn{2}{c}{Weather} &  \multicolumn{2}{c}{Electricity} &  \multicolumn{2}{c}{Traffic}&  \multicolumn{2}{c}{ILI}\\
		\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
		\multicolumn{1}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{1}{*}{96 (24)} & 0.08 & 0.20 & 0.26 & 0.25 & 1.59 & 0.95 & 2.72 & 1.08 & 6.59 &
1.70\\
\multirow{1}{*}{192 (32)} & 0.17 & 0.29 & 0.31 & 0.29 & 1.60 & 0.95 & 2.76 & 1.09 & 7.51 & 1.86\\
\multirow{1}{*}{336 (48)} & 0.31 & 0.40 & 0.38 & 0.34 & 1.62 & 0.96 & 2.79 & 1.10 & 6.58 & 1.80\\
\multirow{1}{*}{720 (64)} & 0.82 & 0.68 & 0.47 & 0.39 & 1.65 & 0.98 & 2.81 & 1.10 & 5.91 & 1.69\\
\bottomrule
	\end{tabular}}
    \label{table:last_value_forecasting}
\end{table} 

==> tables_rebuttal/new_baselines.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{4.9pt}
\scriptsize	
	\centering
	\caption{Comparison of the MSE and MAE results for our proposed multi-scale framework version of Reformer, Performer, and FEDformer  (-\textbf{MSA}) with their original models as the baseline. Results are given in the \emph{multi-variate} setting, for different lenghts of the horizon window. The look-back window size is fixed to $96$ for all experiments. The best results are shown in \textbf{Bold}. Our method outperforms vanilla versions of both Informer and Autoformer over almost all datasets and settings.}
	\scalebox{1.05}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
		\toprule
		\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Reformer-\textbf{MSA}} & \multicolumn{2}{c}{Performer} &  \multicolumn{2}{c}{Performer-\textbf{MSA}} &  \multicolumn{2}{c}{FEDformer} & \multicolumn{2}{c}{FEDformer-\textbf{MSA}}\\
		\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
		\multicolumn{2}{c}{Metric} & MSE & MAE & MAE & MSE & MAE & MAE & MSE & MAE & MSE & MAE & MSE & MAE\\ 
\midrule
\multirow{4}{*}{Exchange} 
 & 96 & 1.063 & 0.826 & \textbf{0.182} & \textbf{0.311} & 0.667 & 0.669 & \textbf{0.179} & \textbf{0.305} & 0.159 & 0.289 & \textbf{0.134} & \textbf{0.264} \\ 
 & 192 & 1.597 & 1.029 & \textbf{0.375} & \textbf{0.446} & 1.339 & 0.904 & \textbf{0.439} & \textbf{0.486} & 0.274 & 0.383 & \textbf{0.259} & \textbf{0.367} \\ 
 & 336 & 1.712 & 1.070 & \textbf{0.605} & \textbf{0.591} & 1.081 & 0.844 & \textbf{0.563} & \textbf{0.577} & \textbf{0.452} & \textbf{0.498} & 0.738 & 0.607 \\ 
 & 720 & 1.918 & 1.160 & \textbf{1.089} & \textbf{0.857} & \textbf{0.867} & \textbf{0.766} & 1.219 & 0.882 & 1.156 & 0.833 & \textbf{0.988} & \textbf{0.792} \\ 
\midrule
\multirow{4}{*}{Weather} 
 & 96 & 0.347 & 0.388 & \textbf{0.199} & \textbf{0.263} & 0.441 & 0.479 & \textbf{0.228} & \textbf{0.291} & 0.292 & 0.370 & \textbf{0.225} & \textbf{0.287} \\ 
 & 192 & 0.463 & 0.469 & \textbf{0.294} & \textbf{0.355} & 0.475 & 0.501 & \textbf{0.302} & \textbf{0.357} & 0.375 & 0.428 & \textbf{0.331} & \textbf{0.382} \\ 
 & 336 & 0.734 & 0.622 & \textbf{0.463} & \textbf{0.464} & 0.478 & 0.482 & \textbf{0.441} & \textbf{0.456} & \textbf{0.455} & 0.473 & 0.460 & \textbf{0.458} \\ 
 & 720 & 0.815 & 0.674 & \textbf{0.493} & \textbf{0.471} & \textbf{0.563} & \textbf{0.552} & 0.817 & 0.655 & \textbf{0.640} & 0.573 & 0.697 & \textbf{0.564} \\ 
\midrule
\multirow{4}{*}{Electricity} 
 & 96 & 0.294 & 0.382 & \textbf{0.183} & \textbf{0.291} & 0.294 & 0.387 & \textbf{0.190} & \textbf{0.300} & 0.202 & 0.317 & \textbf{0.180} & \textbf{0.296} \\ 
 & 192 & 0.331 & 0.409 & \textbf{0.194} & \textbf{0.304} & 0.305 & 0.400 & \textbf{0.200} & \textbf{0.310} & 0.200 & 0.313 & \textbf{0.187} & \textbf{0.301} \\ 
 & 336 & 0.361 & 0.428 & \textbf{0.209} & \textbf{0.321} & 0.331 & 0.416 & \textbf{0.209} & \textbf{0.322} & 0.213 & 0.329 & \textbf{0.206} & \textbf{0.322} \\ 
 & 720 & 0.316 & 0.393 & \textbf{0.234} & \textbf{0.340} & 0.304 & 0.386 & \textbf{0.228} & \textbf{0.335} & \textbf{0.236} & 0.348 & 0.239 & \textbf{0.347} \\ 
\midrule
\multirow{4}{*}{Traffic} 
 & 96 & 0.698 & 0.386 & \textbf{0.615} & \textbf{0.377} & 0.730 & 0.405 & \textbf{0.612} & \textbf{0.371} & 0.596 & 0.373 & \textbf{0.564} & \textbf{0.349} \\ 
 & 192 & 0.694 & 0.378 & \textbf{0.613} & \textbf{0.367} & 0.698 & 0.387 & \textbf{0.608} & \textbf{0.368} & 0.599 & 0.372 & \textbf{0.569} & \textbf{0.347} \\ 
 & 336 & 0.695 & 0.377 & \textbf{0.617} & \textbf{0.360} & 0.678 & 0.370 & \textbf{0.604} & \textbf{0.356} & 0.600 & 0.374 & \textbf{0.576} & \textbf{0.347} \\ 
 & 720 & 0.692 & 0.376 & \textbf{0.638} & \textbf{0.360} & 0.672 & 0.364 & \textbf{0.634} & \textbf{0.360} & 0.612 & 0.374 & \textbf{0.601} & \textbf{0.360} \\ 
\bottomrule
	\end{tabular}}
    \label{table:new_baselines}
\end{table} 
